The viscous evolution of circumstellar discs in young star clusters

Stars with circumstellar disks may form in environments with high stellar and gas densities which affects the disks through processes like truncation from dynamical encounters, ram pressure stripping, and external photoevaporation. Circumstellar disks also undergo viscous evolution which leads to disk expansion. Previous work indicates that dynamical truncation and viscous evolution play a major role in determining circumstellar disk size and mass distributions. However, it remains unclear under what circumstances each of these two processes dominates. Here we present results of simulations of young stellar clusters taking viscous evolution and dynamical truncations into account. We model the embedded phase of the clusters by adding leftover gas as a background potential which can be present through the whole evolution of the cluster, or expelled after 1 Myr. We compare our simulation results to actual observations of disk sizes, disk masses, and accretion rates in star forming regions. We argue that the relative importance of dynamical truncations and the viscous evolution of the disks changes with time and cluster density. Viscous evolution causes the importance of dynamical encounters to increase in time, but the encounters cease soon after the expulsion of the leftover gas. For the clusters simulated in this work, viscous growth dominates the evolution of the disks.

==> tex/results_table.tex <==
\begin{table*}
\centering
\bgroup
\def\arraystretch{1.2}%
\begin{tabular}{c|ccccc}
                                     & Trapezium  & Lupus clouds                                                                & Chamaeleon I & $\sigma$ Orionis & Upper Scorpio \\
\hline \hline
Obtained best fit $N$          &  750          & 1000                                                                             &      25        &      25            &   25      \\ \hline
Obtained best fit $\alpha$  &   $\num{e-2}$     &      $\num{e-4}$      & $\num{e-4}$                                                                    &        $\num{e-4}$      &         $\num{2e-3}$     \\ \hline
Obtained best fit $\rho_N$ (stars $pc^{-3}$)     &   1816.09         & 509.35 &    35.25          &       35.25         &         35.25     
\end{tabular}
\egroup
\caption{Obtained best fits for the observed clusters.}\label{results_table}
\end{table*}
